Snowmass '21 Community Engagement Frontier 6: Public Policy and Government Engagement: Congressional Advocacy for HEP Funding (The "DC Trip'')

This document has been prepared as a Snowmass contributed paper by the Public Policy \& Government Engagement topical group (CEF06) within the Community Engagement Frontier. The charge of CEF06 is to review all aspects of how the High Energy Physics (HEP) community engages with government at all levels and how public policy impacts members of the community and the community at large, and to assess and raise awareness within the community of direct community-driven engagement of the U.S. federal government (\textit{i.e.} advocacy). The focus of this paper is the advocacy undertaken by the HEP community that pertains directly to the funding of the field by the U.S. federal government.

==> Deprecated/big_picture_questions.tex <==
\include{Sections/big_picture}
\begin{comment}
\outline{
\begin{itemize}
    \item HEP leadership in science advocacy
    \begin{itemize}
        \item HEP is well-poised to lead the US science community in advocating for infrastructural change to how science is funded because (1) we are good at advocacy and (2) we have the advantage of doing ``big science''
    \end{itemize}
    \item Currently go to congress and ask for funding year after year to prevent erosion of our funding. Is there room to also ask for a change in the way HEP is funded?
    \begin{itemize}
        \item More funding is part of this, but not really a solution.
        \item Should scientists be more present when conversations about science funding take place? (e.g. DOE/NSF for the Future in the House, Endless Frontier in the Senate) 
        \begin{itemize}
            \item Learn from history: putting a lot of new funding into a specific research area (nanotechnology, AI/ML, quantum, \ldots) often does not actually advance that effort, because funding for other areas is always getting cut, and scientists try to maintain their labs/research groups by rephrasing existing research to fit new funding calls
        \end{itemize}
        \item Can we advocate for different ways of doing science funding? Can we do it without tearing down the existing system until we’re ready?
        \item Can we look to ARPA type proposals?
        \item One idea:
        \begin{itemize}
            \item Make it easy to apply for \$10k. If you do well, then give the opportunity to apply for \$20k, etc. (bootstrap)
            \begin{itemize}
                \item Supplements existing policies about X\% of funding going to under-represented institutes: they still have to deal with large amounts of bureaucracy (which requires specialized expertise and effort) to get that funding
            \end{itemize}
            \item Another idea:
            \begin{itemize}
                \item Continuity of funding for projects (i.e. appropriate funding for multiple years).
                \item  Is this a huge ask? Are there precedents?
            \end{itemize}
        \end{itemize}
    \end{itemize}
    \item Some of these issues go beyond HEP
    \begin{itemize}
        \item Try to spark a bigger conversation/effort
        \item HEP can lead: advocacy experience and success, Big Science projects
    \end{itemize}
    \item Contact Lewis/Burke to ask about how new policies would be implemented in bills, etc.?
    \begin{itemize}
        \item How much freedom do funding agencies have to make changes w/out modifying federal law? 
        \begin{itemize}
            \item E.g. valuing outreach (or inreach) work for merit of grant applications
            \begin{itemize}
                \item Along the lines of data preservation
                \item DEI statements? --- When something is mandatory, people find ways to say they’re doing things without actually doing them\ldots may not help as much in the long run
            \end{itemize}
        \end{itemize}
        \item DOE vs. NSF work differently
        \item Appropriate funds for more than 1 year at a time: Europe does this, US doesn’t, decreases international trust in US-led/-based efforts
    \end{itemize}
    \item We think that there’s a bit of an optics issue when it comes to the DOE’s role in the public (and elected officials') eye when it comes to thinking about how science in the US is funded. (Per Alan Stone,) the DOE funds 85\% of USHEP. Is this worth pointing out? It’s not clear what, if anything, can be done about this.
\end{itemize}}
\end{comment}

==> Deprecated/history.tex <==
The annual community activities evolved over more than 35 years to reach where they are today. The trip was started by a small number of scientists who were part of the Fermilab Users Executive Committee, and grew to involve scientists from the SLAC Users Executive Committee \href{https://www-group.slac.stanford.edu/sluo/}{SLUO} which formed in 1989, but has been last active in the last 10 years. The Fermilab Users Executive Committee UEC represents the XXX Users at the lab, and SLUO 



US LUA signed an agreement with URA in May 2013, and was registered by DC.gov as a
nonprofit association registered in Washington DC as of June 6, 2013, based at URA headquarters.
As an independent Association, USLUA relies on the contributions of its membership.
USLUA is a nonprofit, tax exempt organization recognized under section 501(c)(3) of the US
Internal Revenue Code, federal ID #54-1827596. All contributions to USLUA are tax deductible.





\begin{comment}
    \item  Herman has been emailed 
    \item This would be a good place to explain how it came to be that the current leading organisations are the ones that they are
    \item How trip responded to last P5 - ask Breese Quinn? 
\end{comment}

==> Notes/contributors.tex <==
\section{Contributors}
Below is a list of people who have confirmed interest in contributing to the white paper:

John Orrell, 
Noah Kurinsky, 
Yoni Kahn, 
Richard Schnee, 
Rouven Essig, 
Alexander Kish, 
Claudio Savarese, 
Matthew Szydagis, 
Cristiano Galbiati, 
Isaac Arnquist, 
Chris Jackson, 
Richard Gaitskell, 
Alden Fan, 
Daniel McKinsey, 
Alissa Monte, 
Scott Hertel, 
Scott Haselschwardt, 
Madan Timalsina, 
David Woodward, 
Lauren Hsu, 
Rafael Lang, 
Vetri Velan, 
Maria Laura di Vacri, 
Kim Berghaus, 
Tarek Saab, 
Susana Cebrian, 
Eric Dahl, 
Dylan Temples, 
Jacob McLaughlin, 
Alan Robinson, 
Eric Hoppe, 
Richard Saldanha, 
Anthony Villano, 
Sagar Poudel, 
Ben Loer, 
Karthik Ramanathan, 
Alvaro Chavarria, 
Ian Lawson, 
Enectali Figueroa-Feliciano, 
Jeter Hall, 
Jingke Xu, 
Jacques Pienaar, 
Peizhi Du, 
Daniel Egana-Ugrinovic, 
Mukul Sholapurkar

\textcolor{red}{If you would look to contribute and are not on this list, please email us and ask to be added!}

==> Notes/loisummaries.tex <==
\section*{LOIs relevant to particle DM backgrounds and calibration}

\begin{enumerate}
    \item {\verb SNOWMASS21-CF1_CF0-TF9_TF0_Baxter-112.pdf } $\rightarrow$ Inelastic DM-Nucleon Scattering
    \begin{itemize}
        \item Migdal
        \item collective effects in crystals
        \item low-energy NR calibration
        \item overlap with papers \#2 and \#4
    \end{itemize}
    \item {\verb SNOWMASS21-CF1_CF0_Sumit_Ghosh-119.pdf } $\rightarrow$ Inelastic DM-Nucleon Scattering 
    \begin{itemize}
        \item Migdal
        \item sub-eV phonon response
        \item overlap with papers \#2 and \#4
    \end{itemize}
    \item {\verb SNOWMASS21-IF8_IF0-NF5_NF10-CF1_CF0-CompF5_CompF7_Matthew_Szydagis-104.pdf } $\rightarrow$ NEST
    \begin{itemize}
        \item Detector response models/simulations
        \item overlap with paper \#4
    \end{itemize}
    \item {\verb SNOWMASS21-IF3_IF5-EF1_EF4-183.pdf } $\rightarrow$ TPC development 
    \begin{itemize}
        \item TPC development and calibration
        \item overlap with IF
    \end{itemize}
    \item {\verb SNOWMASS21-IF8_IF0_Shawn_Westerdale_and_Michael_Clark-133.pdf } $\rightarrow$ TPC development 
    \begin{itemize}
        \item TPC development and calibration
        \item modeling electron emission
        \item modeling electric fields
        \item noble gas purification
        \item cosmogenic activation
        \item overlap with IF
    \end{itemize}
    \item {\verb SNOWMASS21-IF8_IF9_Westerdale-141.pdf } $\rightarrow$ TPC development
    \begin{itemize}
        \item NR yield calibrations
        \item overlap with IF
    \end{itemize}
    \item {\verb SNOWMASS21-IF8_IF9-042.pdf } $\rightarrow$ LAr TPC development
    \begin{itemize}
        \item gas purification
        \item overlap with IF
    \end{itemize}
    \item {\verb SNOWMASS21-IF8_IF6_Michael_Mooney-192.pdf } $\rightarrow$ LAr TPC development
    \begin{itemize}
        \item calibration of large detectors
        \item recombination modeling
        \item E field modeling
        \item light/charge yield
        \item overlap with IF and NF
    \end{itemize}
    \item {\verb SNOWMASS21-NF10_NF9-IF6_IF0_PSD_Li-6-Doped_Scintillator-180.pdf } $\rightarrow$ 6Li-doping of Organic Scintillators
    \begin{itemize}
        \item calibration standards
        \item overlap with NF
    \end{itemize}
    \item {\verb SNOWMASS21-NF7_NF6_Samuel_Hedges-153.pdf }$\rightarrow$ Measuring Reactor Neutrinos
    \begin{itemize}
        \item background modeling
        \item overlap with NF
    \end{itemize}

    \item 	{\verb SNOWMASS21-CF1_CF0-IF1_IF0_Rouven_Essig-089.pdf } $\rightarrow$ GaAs for ERDM
    \begin{itemize}
        \item Crystal microfractures, environmental vibrations
        \item Cosmogenic isotopes in GaAs (e.g., tritium)
        \item Photon veto detectors
    \end{itemize}
    %SNOWMASS21-EF-TOPIC0-004.pdf --> hidden sector detectability paper
    %SNOWMASS21-AF5_AF0-NF2_NF0-RF6_RF0_Vandewater-215.pdf --> LANSCE facility improvement for beam-dump experiments
    \item {\verb SNOWMASS21-CF1_CF7-NF5_NF3_PandaX-073.pdf } $\rightarrow$ PandaX (LXe)
    \begin{itemize}
        \item Low background facility $\rightarrow$ DURF (CJPL-II)
        \item Cherenkov photons, low-background photosensors, cosmogenic backgrounds (e.g., Xe-137)
        \item production of clean xenon
    \end{itemize}
    \item {\verb SNOWMASS21-CF1_CF0_Eric_Dahl-099.pdf } $\rightarrow$ SBC (scintillating bubble chamber)
    \begin{itemize}
        \item liquid noble intrinsic backgrounds (e.g., Ar-39)
        \item Low-energy NR ionization yield calibration using photoneutron sources
    \end{itemize}
    \item {\verb SNOWMASS21-CF1_CF0_Jay_Hyun_Jo-263.pdf } $\rightarrow$ NaI (DM-Ice200)
    \begin{itemize}
        \item NaI intrinsic backgrounds:  e.g., tritium, Pb-210, K-40
    \end{itemize}
    %	SNOWMASS21-CF3_CF7_Nilanjan_Banik-207.pdf --> stellar streams
    %	SNOWMASS21-CF6_CF3_Dickinson-257.pdf --> ELT telescope
    % SNOWMASS21-IF1_IF0-CF1_CF2-TF10_TF0-013.pdf  --> mechanical/gravitational sensors (seems very technology specific)
    \item {\verb SNOWMASS21-CF1_CF2-NF3_NF10-IF1_IF0-UF3_UF2_SuperCDMS-077.pdf } $\rightarrow$ SuperCDMS
    \begin{itemize}
        \item backgrounds: H-3, Si-32, Pb-210 (from Rn), leakage current, low-energy secondary emissions
        \item facility needs:  low-radon cleanroom for detector growth, fab (possibly underground)
        \item active veto detectors: neutron and/or photon
        \item radiopure material needs:  cryogenic connectors/cables, copper
    \end{itemize}	
    %	SNOWMASS21-NF3_NF0-RF6_RF0-TF8_TF9_Doojin_Kim-070.pdf --> CEvNS- & beam-type experiments
    \item {\verb SNOWMASS21-NF3_NF9-111.pdf } $\rightarrow$ COHERENT
    \begin{itemize}
        \item Low-radioactivity argon (Ar-39)
    \end{itemize}
    %	SNOWMASS21-NF3_NF0-CF1_CF0-TF8_TF9_Doojin_Kim-032.pdf --> inelastic boosted dark matter
    %	SNOWMASS21-CF3_CF1-TF9_TF8_Vera_Gluscevic,_Kimberly_Boddy-110.pdf --> cosmic probes theory/analysis paper
    \item {\verb SNOWMASS21-CF1_CF2-IF2_IF1_Ben_Mazin-004.pdf } $\rightarrow$ MKID haloscope
    \begin{itemize}
        \item blackbody or other low-energy photon background (e.g., secondary emission)
    \end{itemize}
    \item {\verb SNOWMASS21-TF9_TF0-052.pdf } $\rightarrow$ Theory developments for low-threshold detectors
    \begin{itemize}
        \item calculation and calibration of material properties to understand secondary emission backgrounds (e.g., analytic methods, numerical computation using DFT)
        \item calibration of scattering processes: Migdal, bremsstrahlung, plasmons, de-excitation of metastable nuclear isomers
        \item calibration of collective-mode excitations: phonons, plasmons, magnons
        \item calibration of absorption cross sections (e.g., photo-absorption)
    \end{itemize}
    %	SNOWMASS21-CF3_CF1_Regina_Caputo-121.pdf --> indirect detection
    \item {\verb SNOWMASS21-CF1_CF0_Matthew_Szydagis-174.pdf } $\rightarrow$ G3 LXe
    \begin{itemize}
        \item backgrounds:  pp solar neutrinos, radon, dust
    \end{itemize}
    % SNOWMASS21-CF1_CF3_Georgia_Karagiorgi-170.pdf --> GRAMS (LXe TPC balloon experiment)
    \item {\verb SNOWMASS21-CF1_CF2-IF1_IF2-102.pdf } $\rightarrow$ joint sensitivity of CCDs and KIDs
    \begin{itemize}
        \item backgrounds:  leakage current, low-energy secondary emissions
        \item materials:  ultra-hire-purity silicon
    \end{itemize}
    %	SNOWMASS21-CF3_CF1_Stefano_Profumo-007.pdf --> GECCO (indirect detection)
    %	SNOWMASS21-CF1_CF3_Perez-137.pdf --> GAPS (indirect detection)
    % SNOWMASS21-NF3_NF0-CF1_CF0-TF8_TF9_Doojin_Kim-049.pdf --> boosted DM with surface neutrino detectors
    \item {\verb SNOWMASS21-IF1_IF0-NF10_NF0-CF1_CF2_Golwala-080.pdf } $\rightarrow$ cryogenic phonon-mediated MKID detectors
    \begin{itemize}
        \item instrumental/environmental backgrounds:  vibrations, blackbody/RF power, etc.
    \end{itemize}
    %	SNOWMASS21-IF9_IF8-NF3_NF10-CF1_CF0-145.pdf --> direction detection with dual-readout TPC ion tracking
    %	SNOWMASS21-IF8_IF2_Andrzej_Szelc-145.pdf --> wavelength shifting reflectors for neutrino detectors
    %	SNOWMASS21-CF7_CF0-EF6_EF7-NF5_NF6-AF4_AF0_LAA-074.pdf --> complementarity of asatroparticle & colliders
    %	SNOWMASS21-NF1_NF4_Pedro_Ochoa-034.pdf --> JUNO (indirect detection)
    %   SNOWMASS21-NF2_NF3-RF6_RF0_Athanasios_Hatzikoutelis-160.pdf --> beam-based experiments
    %	SNOWMASS21-NF9_NF5-CF1_CF0-IF8_IF0_JNewby-108.pdf --> facility for accelerator-produced DM
    \item {\verb SNOWMASS21-NF5_NF4-084.pdf } $\rightarrow$ DARWIN (LXe)
    \begin{itemize}
        \item backgrounds:  Rn-222, Kr-85 (intrinsic)
        \item materials:  radiopure titanium
    \end{itemize}
    %	SNOWMASS21-NF4_NF3_Matthew_Strait-090.pdf --> NOVA
    %	SNOWMASS21-IF2_IF8-NF10_NF0_Gramellini-137.pdf --> multi-modal pixels (detector tech)
    %	SNOWMASS21-IF8_IF0-NF10_NF6_Jacob_Zettlemoyer-150.pdf --> directional detection
    %	SNOWMASS21-NF-TOPIC0-001.pdf --> CONNIE (neutrino detector
    \item {\verb SNOWMASS21-NF10_NF4-CF1_CF0-IF8_IF0-UF1_UF3-137.pdf } $\rightarrow$ kTon-scale LAr
    \begin{itemize}
        \item materials:  low-radioactivity argon, general background control (material radiopurity)
        \item backgrounds:  Ar-39, Ar-42, radon
    \end{itemize}
    %	SNOWMASS21-NF3_NF4_Russell_Neilson-017.pdf --> SBC again
    %	SNOWMASS21-NF3_NF2-CF7_CF1-TF9_TF8_Katori-073.pdf --> IceCube (indirect)
    %	SNOWMASS21-NF8_NF4-CF1_CF7_Evan_Grohs-174.pdf --> sort of a phenomenology LOI (cosmolgocial neutrinos)
    \item {\verb SNOWMASS21-NF4_NF3-CF1_CF7-TF9_TF11-039.pdf } $\rightarrow$ astrophysical neutrinos
    \begin{itemize}
        \item calibration/characterization of neutrino backgrounds:  solar, atmospheric, supernova
    \end{itemize}

    \item {\verb SNOWMASS21-CF1_CF2-RF0_RF0-155.pdf }$\rightarrow$ BSM Searches with the LEGEND Double Beta Decay Experiment
    \begin{itemize}
        \item Backgrounds for LEGEND's BSM dark matter program include Ar-39, Ar-42, and cosmogenic tritium and Ge-68
    \end{itemize} 
	\item {\verb SNOWMASS21-CF1_CF0-IF8_IF0_Guillaume_Giroux-085.pdf } $\rightarrow$ Search for Low Mass WIMPs with Spherical Proportional Counters
	\begin{itemize}
	    \item NEWS-G search for 0.1-10 GeV WIMPs with low-A gasses requires low-radioactivity Cu in low-Pb-210 archaeological Pb shield
	    \item Main background from Pb-210 in Cu (Bremsstrahlung photons from Bi-210 beta decay)
	    \item Future iterations will use 6N electroformed Cu for better purity
	\end{itemize}
	\item {\verb SNOWMASS21-RF3_RF0-CF2_CF0-IF1_IF0_Andrew_Geraci-076.pdf } $\rightarrow$ Optically levitated sensors for precision tests of fundamental physics
	\begin{itemize}
	    \item This may require a novel calibration scheme
	    \item Backgrounds are likely different than for other searches
	\end{itemize}
	\item {\verb SNOWMASS21-IF9_IF8-NF3_NF10-CF1_CF0-145.pdf } $\rightarrow$ Dual-Readout Time Projection Chamber:exploring sub-millimeter pitch for directional dark matter and tau identification in $\nu_\tau$ CC interactions 
	\begin{itemize} 
	\item Direction-sensitive DD with noble gas TPCs, will need NR/angular reoslution calibration
	\end{itemize}
	\item {\verb SNOWMASS21-IF2_IF0-CF0_CF1_JUIJEN_WANG-132.pdf } $\rightarrow$ Transparent Thermoplastic Acrylic Scintillator 
	\begin{itemize}
	    \item Acrylic scintillators for neutrinos and DM, radiopure acrylic is important
	    \item Presumably need to calibrate scintillation efficiency with different dopants (e.g. napthalene)
	    \item Rn daughter plateout is a significant concern
	\end{itemize}
	\item {\verb SNOWMASS21-UF4_UF3-NF5_NF6-CF1_CF0-IF3_IF0-CompF2_CompF3-CommF5_CommF0-006.pdf } $\rightarrow$ Advanced Germanium Detectors and Technologies for Underground Physics
	\begin{itemize}
	    \item Very low threshold Ge detectors for LDM and neutrinos, target threshold 0.7 eV to 100 eV
	    \item Target background rate $<1\times10^{-5}$\,cts/keV/kg/yr
	    \item Need to calibrate charge and phonons
	    \item Needs underground crystal growth
	    \item Backgrounds from leakage current, electrical breakdown, electronics
	    \item Needs sub-keV NR calibration, testing (n,$\gamma$) calibration
	\end{itemize} 
	\item {\verb SNOWMASS21-CF1_CF0-079.pdf } $\rightarrow$ Multi-ton scale bubble chambers
	\begin{itemize}
	    \item PICO, at a tonne-scale, has eliminated backgrounds from metastable particle-born water droplets
	    \item Needs $<5$\,nBq/m$^2$ of surface $\alpha$ activity to avoid pileup
	    \item Needs low-background active fluid containers other than fused silica to scale up
	    \item Has efficient vetoing of muon-induced backgrounds
	\end{itemize}
	\item {\verb SNOWMASS21-CF1_CF0_Claudio_Savarese-125.pdf } $\rightarrow$ Silicon Photomultipliers as a target for low-mass dark matter searches
	\begin{itemize}
	    \item Low-background SiPMs can serve as low-mass DM detectors with 150 eV thresholds in a LNe veto
	    \item Main backgrounds from DCR  and DiCT
	    \item Main R\&D challenge is to minimize cross-talk, reduce Si-32
	    \item Need low-noise, low-background electronics
	    \item Most $\gamma$'s and $\alpha$'s will be vetoed, need to reduce those that aren't
	\end{itemize}
	\item {\verb SNOWMASS21-IF1_IF8-CF1_CF0_Hertel-158.pdf } $\rightarrow$ Calorimetric readout of a superfluid 4He target mass
	\begin{itemize}
	    \item SHe detector, needs NR calibration down the the meV scale
	    \item Needs ER calibration down to 19.8 eV
	\end{itemize}
	\item {\verb SNOWMASS21-IF1_IF2-CF1_CF0-182.pdf } $\rightarrow$ Improving the Sensitivity of Athermal Phonon Sensors for Light Mass Dark Matter
	\begin{itemize}
	    \item Phonon sensors for light DM, need NR and ER calibration down to the O(100 meV) scale
	    \item Backgrounds from dark counts, leakage current, and environmental vibraitons
	\end{itemize} 
	\item {\verb SNOWMASS21-CF1_CF0_Giovanetti-172.pdf } $\rightarrow$ Searching for Dark Matter with Liquid Argon
	\begin{itemize}
	    \item GADMC needs to reduce Ar-39 and Kr085, which it will do with Urania UAr extraction plant and Aria purification column
	    \item Needs low-background SiPMs
	    \item Backgrounds from neutrons, reduced with veto
	    \item DarkSide-LowMass will target < 50\,8Bq/kg of Ar-39
	    \item Backgrounds from the neutrino floor
	\end{itemize}
	\item {\verb SNOWMASS21-IF8_IF0_Shawn_Westerdale_and_Michael_Clark-133.pdf } $\rightarrow$ R\&D for low-threshold noble liquid detectors
	\begin{itemize}
	    \item Low-threshold noble liquid detectors will need sub-keV ER and NR calibration
	    \item Need to understand and reduce spurious electron backgrounds
	    \item Radiopurity constraints to minimize ER backgrounds, Kr-85, Ar-39, tritium, Rn-220, Rn-222, radiopure SiPMs and other materials
	    \item Need high chemical purity for target
	    \item Need to understand cosmic ray activation of target and materials (significant uncertainties) and low-energy beta spectra uncertainties
	\end{itemize} 
	\item {\verb SNOWMASS21-IF8_IF0_Eric_Dahl-135.pdf } $\rightarrow$ Enabling the next generation of bubble-chamberexperiments for dark matter and neutrino physics
	\begin{itemize}
	    \item SBC needs vessel materials that won't induce nucleation
	    \item NR threshold calibration vs. ER nucleation rate as a function of superheat
	    \item Scintillation response calibration $\sim10$\,keV 
	    \item What Ar-39 background rate can they sustain?
	\end{itemize}
	\item {\verb SNOWMASS21-IF1_IF0-CF1_CF0_Marshall-110.pdf } $\rightarrow$ Solid-state directional detection of massive dark matterparticles via spectroscopy of quantum defects
	\begin{itemize}
	    \item Large bandgap directional DM detectors like diamond and silicon carbide need ER/NR calibration down to 1--3 keV with angular resolution calibration 
	    \item Need underground facilities to avoid cosmic ray exposure of crystals during creation or post-run track/damage analysis
	\end{itemize}
	\item {\verb SNOWMASS21-CF1_CF0-IF1_IF2_Rouven_Essig-075.pdf } $\rightarrow$ Direct Detection of Spin-independent and Spin-dependent Nuclear Scattering of Sub-GeV Dark Matter Using Molecular Excitations and Superconducting Nanowire Single-Photon Detectors
	\begin{itemize}
	    \item Superconducting Nanostrip Single-Photon Detectors will require ER and NR calibration below 100\,meV
	\end{itemize}
	\item {\verb SNOWMASS21-IF2_IF0-CF3_CF4_Drlica-Wagner-021.pdf } $\rightarrow$ Skipper CCDs for Cosmic Surveys of Dark Energy and Dark Matter
	\begin{itemize}
	    \item Direct detection with skipper CCDs requires low-background and low-noise readout electronics
	\end{itemize}
	\item {\verb SNOWMASS21-CF1_CF0-IF2_IF0_Juan_Estrada-080.pdf } $\rightarrow$ Status and plans for Oscura: A Multi-kilogram Skipper-CCD Array forDirect-Detection of Dark Matter
	\begin{itemize}
	    \item Needs low-background, low-noise electronics readout
	    \item Targeting 0 ionization events in the 2--10\,electron range
	    \item Need to mitigate cosmogenic activation and ensure highly radipure material selection
	\end{itemize}
	\item {\verb SNOWMASS21-CF1_CF2_Baudis-114.pdf } $\rightarrow$ Dark matter physics with the DARWIN Observatory
	\begin{itemize}
	    \item DARWIN needs to achieve $10^{-3}$ ER rejection at 50\% NR acceptance
	    \item Backgrounds from the neutrino floor
	    \item Uses a veto to reject neutron backgrounds 
	    \item Kr-85 and Rn-220 removal is important 
	    \item Requires NR and ER calibration systems
	\end{itemize}
	\item {\verb SNOWMASS21-CF1_CF2-NF5_NF4-IF8_IF0-CompF0_CompF0-UF2_UF3_Matthew_Szydagis-236.pdf } $\rightarrow$ The Exploitation of Xe Large Scale Detector Technology for a Range of Future Rare Event Physics Searches
	\begin{itemize}
	    \item Future large Xe detectors will need calibration down to O(10 eV)
	    \item Need to reduce single- and few-electron backgrounds
	    \item Need to reduce Kr-85 and Rn-220 backgrounds
	\end{itemize}
	\item {\verb SNOWMASS21-RF0_RF0-EF0-CF1-IF0_Jiansong_Gao-086.pdf } $\rightarrow$ Million-pixel Kinetic Inductance Detector Arrays for sub-GeV Light Dark Matter Search
	\begin{itemize}
	    \item Dark matter detection with MKIDS
	    \item Background discrimination between DM events and substrate events
	    \item Requires O(100 meV) calibration
	    \item Use veto for backgorund discrimination 
	\end{itemize}

\item {\verb SNOWMASS21-NF7_NF9-IF8_IF0_Kaixuan_Ni-011.pdf } $\rightarrow$ Noble Liquids for the Detection of CE$\nu$NS from Artificial Neutrino Sources 
\begin{itemize}
\item Accurate CEvNS background modelling using large statistics from artificial neutrino sources 
\item Calibration of sub-keV nuclear recoils using neutrinos 
Detector: 100-kg scale compact dual-phase Ar or Xe near neutrino sources
\end{itemize}
\
\item {\verb SNOWMASS21-IF8_IF0-CF1_CF0_Dongqing_Huang-152.pdf $\rightarrow$ Charcoal-based Radon Reduction Systems for Ultra-clean Rare-event Detectors}
\begin{itemize}
    \item Radon dominant in G2. For G3, radon reduction an entire circulation loop at high flow rate is necessary. Could modify vacuum swing adsorption systems so that they can return noble carrier gases to the purification system through a gas feedback loop. 
    \item Develop ultra-low radon emanating adsorbents with intrinsic radon activity about a factor of 2.5 or better
\end{itemize}

\item {\verb SNOWMASS21-EF9_EF10-NF3_NF0-RF6_RF0-AF5_AF0-IF3_IF7_MATHUSLA_(David_Curtin)-184.pdf $\rightarrow$ Recent Progress and Next Steps for the MATHUSLA LLP Detector}
\begin{itemize}
    \item Progress in detailed background simulations of upward going muons, cosmic rays and atmospheric neutrinos - most are vetoed
\end{itemize}

\item {\verb SNOWMASS21-TF9_TF10-CF1_CF2_Zhengkang_Zhang-081.pdf $\rightarrow$ Light dark matter direct detection at the interface with condensed matter physics}
\begin{itemize}
\item Interdisciplinary theoretical research needed to accurately compute signal and background processes for non-WIMP DM. Calculations of material responses to DM interactions are needed, with a combination of analytic and numerical tools.
\end{itemize}

\item {\verb SNOWMASS21-IF8_IF0-CF1_CF0_sorensen-053.pdf $\rightarrow$ A crystalline future for dual phase xenon direct detection instruments}
\begin{itemize} 
\item could potentially offer near-total mitigation of radon backgrounds
\end{itemize}

\item {\verb SNOWMASS21-CF1_CF0-NF5_NF0-RF4_RF0-AF5_AF0-IF9_IF0_Shawn_Westerdale-052.pdf  $\rightarrow$ Neutron yield in $(\alpha, n)$-reactions in rare-event searches }
\begin{itemize}
\item Important for calculating expected NR backgrounds from neutrons 
\item unite nuclear and particle physicists interested in $(\alpha, n)$ reactions, including $(\alpha, n\gamma)$, in order to improve $(\alpha, n)$ yield and neutron spectrum calculations
\end{itemize}
\item {\verb SNOWMASS21-IF1_IF2_Gianpaolo_Carosi-179.pdf $\rightarrow$ Effects of Energy Accumulation and Avalanche-like Releases in Materials and Low Energy Threshold Detectors}
\begin{itemize}
\item Trying to explain low energy background excesses in multiple detectors (rising background as energy decreases). Study proposed to look for “hot photons” in SNSPDs
\end{itemize}

\item{\verb SNOWMASS21-CF1_CF0_Hugh_Lippincott-106.pdf	 $\rightarrow$ HydroX- Using hydrogen doped in liquid xenon to search for dark matter} 
\begin{itemize}
    \item Will need low energy calibration
\end{itemize}

\item{\verb SNOWMASS21-IF1_IF2-CF1_CF0-147.pdf	 $\rightarrow$ HydroX- Superconducting Nanowire Single-Photon Detector}
\begin{itemize}
    \item the SNSPD is much less sensitive to background counts due to energy deposited into the substrate and coupling into the device.
\end{itemize}
\item {\verb SNOWMASS21-EF9_EF0-NF3_NF0-RF6_RF0_Matthew_Citron-072.pdf $\rightarrow$ Sensitivity reach of scintillation-based detectors for millicharged particles} 
\begin{itemize}
    \item the SNSPD is much less sensitive to background counts due to energy deposited into the substrate and coupling into the device. 
\end{itemize}
 \item {\verb SNOWMASS21-EF9_EF0-NF3_NF0-RF6_RF0_Matthew_Citron-072.pdf $\rightarrow$ Sensitivity reach of scintillation-based detectors for millicharged particles}
 \begin{itemize}
     \item  milliQan used to investigate backgrounds to detectors looking for millicharged particle from LHC collisions
 \end{itemize}
\item {\verb SNOWMASS21-IF1_IF9-CF1_CF2-UF2_UF5-124.pdf $\rightarrow$ Coupling Experiment and Simulation to Model Non-Equilibrium Quasiparticle Dynamics in Superconductors}
\begin{itemize}
    \item Help model noise backgrounds for low threshold searches
\end{itemize}
\item {\verb SNOWMASS21-CF1_CF2-NF3_NF10-IF1_IF0-UF3_UF2_SuperCDMS-077.pdf $\rightarrow$
A Strategy for Low-Mass Dark Matter Searches with Cryogenic Detectors in the SuperCDMS SNOLAB Facility }
\begin{itemize}
    \item Reduce $^{210}$Pb surface backgrounds: sidewall etching, fabrication in a low-radon cleanroom
    \item Reduce apparatus  background: (materials sourcing)
    \item Reduce $^{32}$Si background: isotopic enrichment,
    \item Reduce $^{3}$H background: crystal growth, crystal preparation, detector fabrication, and detector testing all underground
    \item Calibration: Extend NR discrimination to lower recoil energy: Improve ionization resolution for ionization-yield-based discrimination, improve phonon energy resolution 
\end{itemize}
\item {\verb SNOWMASS21-IF8_IF0-UF3_UF0_Brian_Mong-144.pdf $\rightarrow$ Using Metal Organic Frameworks for Krypton and Radon Removal in Low-Background Xenon Detectors}
  \begin{itemize}
  \item Use MOF to separate Kr and Rn from xenon in detectors 
    \item Additionally, MOF may be a way to improve radon removal systems used to provide radon free clean spaces to build low background detectors
  \end{itemize}
\item {\verb SNOWMASS21-UF0_UF0-NF10_NF5-CF1_CF0-IF9_IF0-006.pdf $\rightarrow$ An Ultralow Background Facility to Support Next Generation Rare Event Physics Experiments}
\begin{itemize}
\item Propose new facility - centralized management “hub” enabling collaboration, “spokes” would be institutions with unique capabilities 
\item Large scale assays, new backgrounds, cataloging and sharing, understanding and measuring secular disequilibrium, next-generation radon assays 
\end{itemize}
\item {\verb SNOWMASS21-IF8_IF9_Giovanetti-163.pdf $\rightarrow$ Applications for Underground Argon}
\begin{itemize}
    \item Underground extraction and purification of underground argon, which is depleted in $^{39}$Ar
\end{itemize}
\item {\verb SNOWMASS21-UF6_UF4-NF5_NF0-CF1_CF0_Tim_Sumner-003.pdf $\rightarrow$ Development of the Boulby Underground Laboratory in the UK into a facility to host major international rare event searches. }
\begin{itemize}
    \item New low background facility, possible deeper location
\item Existing radioassay suite
\end{itemize}
\item {\verb SNOWMASS21-CompF3_CompF2-NF1_NF5-CF1_CF2-IF8_IF3_Monzani-084.pdf $\rightarrow$ The Future of Machine Learning in Rare Event Searches}
\begin{itemize}
\item Anomaly finding may help with difficult-to-model backgrounds 
\item Improvements in background rejection have been demonstrated using simple neural networks and boosted decision trees
\end{itemize}
\item {\verb SNOWMASS21-CompF2_CompF0_Diamond-014.pdf $\rightarrow$ Simulations of Low-Energy Crystal Physics for Dark Matter Detectors}
\begin{itemize}
    \item Simulation of charge transport, low energy processes, optical diffractive transport etc \& nuclear recoil yield. 
\end{itemize}
\item {\verb SNOWMASS21-CompF2_CompF1-NF1_NF5-CF1_CF2-IF8_IF2_Monzani-085.pdf $\rightarrow$ Fast Simulations for Noble Liquid Experiments} 
\begin{itemize}
\item For large scale Monte Carlo background production
\end{itemize}
\end{enumerate}


==> Notes/notes.tex <==
\section{Notes}
% \textbf{Contact us:} Dan Baxter (dbaxter9@fnal.gov), Ray Bunker (raymond.bunker@pnnl.gov), Sally Shaw (sallyshaw@ucsb.edu), Shawn Westerdale (shawest@princeton.edu)
% \newline\newline

% \textbf{Meeting minutes:} \href{https://docs.google.com/document/d/1gWU_u0ein3faUUeMhZL2AXSJ1Fae-dfCvZ_6NHB_05I/edit?usp=sharing}{https://docs.google.com/document/d/1gWU\_u0ein3faUUeMhZL2AXSJ1Fae-dfCvZ\_6NHB\_05I/edit?usp=sharing}
% \newline\newline


This section is just for taking organizational notes, and will eventually be removed.

\subsection{Contributors}
These are the people who listed themselves as being interested in contributing (just copied from the Google Doc)
\begin{enumerate}
    \item Isaac Arnquist
    \item Rouven Essig (confirms interest, low-threshold DD backgrounds and calibration)
    \item Alden Fan
    \item Rick Gaitskell
    \item Cristiano Galbiati
    \item Scott Haselschwardt
    \item Scott Hertel
    \item Lauren Hsu (confirms interest)
    \item Chris Jackson
    \item Yoni Kahn
    \item Alexander Kish
    \item Noah Kurinsky
    % \item Ben Loer (no longer interested)
    \item Dan McKinsey
    \item Alissa Monte
    \item John Orrell
    \item Claudio Savarese
    \item Richard Schnee 
    \item Matthew Szydagis (confirms interest)
    \item Madan Timalsina
    \item Vetri Velan (confirms interest)
    \item David Woodward
    \item Rafael Lang (confirms interest)
    \item Sagar Poudel
\end{enumerate}

\subsection{Structure}

\begin{enumerate}
    \item Introduction
    \begin{enumerate}
        \item Introduction/motivation/goals
        \item Executive summary
    \end{enumerate}
    % \item Requirements for different detector types
    % \begin{enumerate}
    %     \item liquid nobles
    %     \item bubble chambers
    %     \item solid state
    % \end{enumerate}
    \item Calibration 
    \begin{enumerate}
        \item Nuclear recoil calibration 
        \begin{enumerate}
            \item In situ
            \item Ex situ, including detection of, e.g., Migdal effect, Bremsstrahlung, etc.
        \end{enumerate}
        \item Electronic recoil calibration at low energies
        \begin{enumerate}
            \item In situ
            \item Ex situ, including detection of, e.g., plasmon resonance
        \end{enumerate}
        \item Coherent excitation calibration at low energies
        \begin{enumerate}
            \item In situ
            \item Ex situ
        \end{enumerate}
        % \item Calibration for indirect detection?
        % \item Detecting low-energy phenomena like Migdal effect, Bremsstrahlung, plasmon resonance, coherent photonuclear scattering
        \item Detector response models/simulations (GEANT4, MCNP, Comsol, NEST, phonon transport)
        \item Anything else for specific detection techniques (e.g. directional detectors, indirect detection)?
    \end{enumerate}
    \item Backgrounds 
    \begin{enumerate}
        \item Astrophysical neutrinos (event generation, rates and spectra)
        \item Cosmogenic neutrons 
        \item Radiogenic neutrons (rate calculations, transport, fast and thermal neutron physics)
        % \item Underground environmental backgrounds (gammas, neutron, Rn and dust in air)
        \item Inactive detector material betas/gammas (e.g. U, Th, Pb210, K40)
        \item Surface contaminants (e.g. dust, Pb210, Po210)
        \item Active bulk contaminants, including, e.g., cosmogenically activated isotopes, intrinsic isotopes, contaminants
        \item Near-threshold phenomena 
        \begin{enumerate}
            \item Spurious electrons in noble liquid TPCs 
            \item Photo-ionization 
            \item Leakage currents 
            \item Microfractures 
            \item Vibrations 
            \item RF-induced pulses
            \item Secondary emission processes
            \item Thermal processes
        \end{enumerate}
        % \item Spurious electron backgrounds (e.g. dark rates, leakage currents, photo-ionization)
        % \item Secondary emission processes
        % \item Instrumental noise (microfractures, vibrations, RF induced pulses)
        \item Anything for indirect detection?
    \end{enumerate}
    \item Facilities
    \begin{enumerate}
        \item Radioassays
        \item Underground material production plants (generalize to include low-activity argon production, e.g.?)
        \item Underground lab backgrounds, including, e.g., radon \& dust mitigation, gammas and neutrons from cavern walls
        \item Software Infrastructure (Radiopurity database, Background Explorer, Assay Request Tool, etc.)
    \end{enumerate}
\end{enumerate}
Call out general needs, rather than getting too deep in the weeds.\\

Potential points of overlap:
\begin{itemize}
    \item LAr TPCs for Cosmic Rays (Tom Shutt - emailed. DSB)
    \item LAr TPCs for neutrinos (DUNE - added below)
    \item 0vBB - NEXT/nEXO/CUPID/LEGEND (Ben Jones - emailed DSB)
    \item Axion searches?
\end{itemize}

\subsection{Letters of Interest of interest}
This is just a list of LOIs that seem relevant for this white paper, and who the listed contact person is
\begin{enumerate}
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-CF1_CF0_Dongqing_Huang-152.pdf}{Nuclear Recoil Calibration Techniques for Dark Matter and Neutrino Experiments}: Rick Gaitskell (Brown University) [gaitskell@brown.edu]
    \item \href{https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF4_NF3-CF1_CF7-TF9_TF11-039.pdf}{Astrophysical neutrinos and dark matter experiments}: Shunsaku Horiuchi (Virginia Tech) [horiuchi@vt.edu], Louis Strigari (Texas AM University) [strigari@tamu.edu]
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-CF1_CF0_Dongqing_Huang-152.pdf}{Charcoal-based Radon Reduction Systems for Ultra-clean Rare-event Detectors}: Wolfgang Lorenzon (University of Michigan) [lorenzon@umich.edu]
    \item \href{https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-NF5_NF0-RF4_RF0-AF5_AF0-IF9_IF0_Shawn_Westerdale-052.pdf}{Neutron Yield in ($\alpha$-n)-reactions in Rare Event Searches}: Shawn Westerdale (INFN Cagliari) [shawest@princeton.edu]
    \item \href{https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-TF9_TF0_Baxter-112.pdf}{Sub GeV DM-Nucleon Scattering via Collective Excitations: The Inelastic Regime}: Dan Baxter (U. Chicago) [dbaxter@kicp.uchicago.edu] (overlap with papers \#2 and \#4)
    \item \href{https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Sumit_Ghosh-119.pdf}{New Opportunities for Low-Mass Dark Matter Direct Detection With Inelastic Scattering}: Sumit Ghosh (Texas A\&M University ) [ghosh@tamu.edu] (overlap with papers \#2 and \#4)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-NF5_NF10-CF1_CF0-CompF5_CompF7_Matthew_Szydagis-104.pdf}{NEST, The Noble Element Simulation Technique: A Multi-Disciplinary Monte Carlo Tool and Framework for Noble Elements}: Vetri Velan (UC Berkeley) [vvelan@berkeley.edu] (overlap with paper \#4)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF3_IF5-EF1_EF4-183.pdf}{Time Projection Chamber R\&D}: Huiron Qi (Institute of High Energy Physics, CAS) (overlap with IF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0_Shawn_Westerdale_and_Michael_Clark-133.pdf}{R\&D for low-threshold noble liquid detectors}: Shawn Westerdale (INFN Cagliari, Princeton) [shawest@princeton.edu] (overlap with IF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF9_Westerdale-141.pdf}{Instrumentation and R\&D for the Global Argon Dark Matter Collaboration}: Shawn Westerdale (INFN Cagliari, Princeton) [shawest@princeton.edu] (overlap with IF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF9-042.pdf}{Investigations of Fundamental Parameters of Liquid Argon for Particle Detection}: Chao Zhang (BNL) [czhang@bnl.gov] (overlap with IF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF6_Michael_Mooney-192.pdf}{Precision Calibration of Large LArTPC Detectors}: Michael Mooney (Colorado State) [mrmooney@colostate.edu] (overlap with IF and NF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF10_NF9-IF6_IF0_PSD_Li-6-Doped_Scintillator-180.pdf}{Neutrino Physics and Nuclear Security Motivations for the Continued Development of Organic Scintillators with Pulse Shape Discrimination Capability and 6Li-doping}: Nathaniel Bowden (LLNL) [nbowden@llnl.gov] and Pieter Mumm (NIST) [hans.mumm@nist.gov] (overlap with NF)
    \item \href{https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF7_NF6_Samuel_Hedges-153.pdf}{Measuring Inelastic Charged- and Neutral-Current Antineutrino-Nucleus Interactions with Reactor Neutrinos}: Samuel Hedges (Duke University) [sch52@phy.duke.edu] (overlap with NF)

    
    
    
    
% == Scan of LOIs relevant to calibration or background
% 
%  Dan Baxter
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Eric_Dahl-099.pdf (SBC: Noble Bubble Chambers)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-CompF6_CompF0_A.B._Balantekin-107.pdf (QIS)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-NF10_NF4-IF3_IF0_Ethan_Brown-034.pdf (Paleo)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-NF3_NF0-TF8_TF9_Yun-Tse_Tsai-261.pdf (LAr/DUNE)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-TF9_TF0_Baxter-112.pdf (inelastic regime)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2_Baudis-114.pdf (Darwin)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-IF1_IF2-102.pdf (KIDs/CCDs)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-IF1_IF8-120.pdf (TESSERACT - LHe/GaAs)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-NF10_NF0-IF2_IF3_Kurinsky-101.pdf (carbon)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-NF5_NF4-IF8_IF0-CompF0_CompF0-UF2_UF3_Matthew_Szydagis-236.pdf (LXe)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF2_CF0_Gray_Rybka-160.pdf (MADMAX - axion!)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF4_CF0_Steven_Kahn-171.pdf (Rubin Observatory)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF4_CF3-IF2_IF0_David_Erskine-009.pdf (cosmic acceleration)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF4_CF6_Jia_Liu-033.pdf (galaxy statistics)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF5_CF6_Adrian_Lee-262.pdf (CMB)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF0-IF4_IF7_Anze_Slosar-028.pdf (PUMA)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF4_Daniel_Masters-138.pdf (Keck)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF4_Jason_Rhodes-047.pdf (Astro)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF4_MoradinezhadDizgah-248.pdf (Line intensity mapping)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF4-178.pdf (Type 1a)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF4-CompF2_CompF0-167.pdf (Astro)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0_Kristi_L_Engel-226.pdf (Cosmic Rays)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-EF6_EF7_YushkovA-130.pdf (Cosmic Rays)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-EF6_EF7-NF5_NF6-AF4_AF0_LAA-074.pdf (collider)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-NF4_NF0-IF10_IF0-118.pdf (Cosmic rays)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF1_EDV-021.pdf (S8)
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF6-031.pdf (POEMMA)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF0_Erik_Shirokoff-187.pdf (KIDs)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF0-CF6_CF0_Jennifer_Marshall-123.pdf (Astro)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF9-NF10_NF6_Mark_Hartz-151.pdf (Water Cherenkov Test Experiment)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF3_IF5-EF1_EF4-183.pdf (TPC R&D)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF6_IF0_Yasar_Onel-049.pdf (Resistive Plate Chambers)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0_Eric_Dahl-135.pdf (PICO)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0_Shawn_Westerdale_and_Michael_Clark-133.pdf (Noble TPCs)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-NF5_NF10-CF1_CF0-CompF5_CompF7_Matthew_Szydagis-104.pdf (NEST)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF6_Michael_Mooney-192.pdf (DUNE)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF9_Westerdale-141.pdf (LAr)
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF9-042.pdf (LAr)
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF10_NF4-CF7_CF1-TF11_TF0_Darren_Grant-105.pdf (IceCube)
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF10_NF9-IF6_IF0_PSD_Li-6-Doped_Scintillator-180.pdf (PROSPECT)
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF2-RF3_RF0-IF1_IF0_Kyle_Leach-055.pdf (BeEST)
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF4_Russell_Neilson-017.pdf (SBC - neutrino)
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF7_NF6_Samuel_Hedges-153.pdf (CEvNS)

% Sally Shaw
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF7_NF9-IF8_IF0_Kaixuan_Ni-011.pdf
%	https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF0_Nelson-078.pdf
%	https://www.snowmass21.org/docs/files/summaries/UF/SNOWMASS21-UF0_UF0-NF10_NF5-CF1_CF0-IF9_IF0-006.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF9-CF2_CF0-AF5_AF0_Vogel-108.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF2_CompF1-NF1_NF5-CF1_CF2-IF8_IF2_Monzani-085.pdf
%	https://www.snowmass21.org/docs/files/summaries/UF/SNOWMASS21-UF0_UF0-NF10_NF5-CF1_CF0-IF9_IF0-006.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF1_CompF3_Andrew_Connolly-045.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF5_CompF7-CF7_CF1_Charles-054.pdf
%	https://www.snowmass21.org/docs/files/summaries/UF/SNOWMASS21-UF0_UF0_Garcia-Sciveres-001.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-CF1_CF0_Dongqing_Huang-152.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-UF3_UF0_Brian_Mong-144.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF2_CompF0_Diamond-014.pdf
%	https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF0-034.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF3_CompF5-CF5_CF0_Andrew_Connolly-051.pdf
%	https://www.snowmass21.org/docs/files/summaries/EF/SNOWMASS21-EF9_EF10-RF6_RF0-TF7_TF8_James_Beacham-201.pdf
%	https://www.snowmass21.org/docs/files/summaries/EF/SNOWMASS21-EF9_EF10-NF3_NF0-RF6_RF0-AF5_AF0-IF3_IF7_MATHUSLA_(David_Curtin)-184.pdf
%	https://www.snowmass21.org/docs/files/summaries/EF/SNOWMASS21-EF10_EF0_Armesto_LHeC_BSM10-180.pdf
%	https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF2_Sean_Tulin-117.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF9-CF1_CF2-UF2_UF5-124.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF3_Zorawar_Wadiasingh-176.pdf
%	https://www.snowmass21.org/docs/files/summaries/TF/SNOWMASS21-TF9_TF10-CF1_CF2_Zhengkang_Zhang-081.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-CF1_CF0_sorensen-053.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF1_C._J._Martoff-092.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF9_Giovanetti-163.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-NF5_NF0-RF4_RF0_RGuenette-086.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-NF5_NF0-RF4_RF0-AF5_AF0-IF9_IF0_Shawn_Westerdale-052.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF5-NF10_NF0_Ben_Jones-070.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF2_Gianpaolo_Carosi-179.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF2_CF0-TF10_TF0-IF1_IF0_Balatsky-170.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF2-CF1_CF0-147.pdf
%	https://www.snowmass21.org/docs/files/summaries/EF/SNOWMASS21-EF9_EF0-NF3_NF0-RF6_RF0_Matthew_Citron-072.pdf
%	https://www.snowmass21.org/docs/files/summaries/CompF/SNOWMASS21-CompF3_CompF2-NF1_NF5-CF1_CF2-IF8_IF3_Monzani-084.pdf
%	https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF0_Torben_Ferber-020.pdf
%	https://www.snowmass21.org/docs/files/summaries/UF/SNOWMASS21-UF6_UF4-NF5_NF0-CF1_CF0_Tim_Sumner-003.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-192.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Hugh_Lippincott-106.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-023.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-019.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF7-TF9_TF0_Julian_Munoz-214.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF7_Kristi_L_Engel-229.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-TF5_TF8-CompF2_CompF0_Pavlos_M._Vranas-166.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-NF3_NF10-IF1_IF0-UF3_UF2_SuperCDMS-077.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF1_Romero-Wolf-024.pdf

% Shawn Westerdale: Do direction sensitive experiments require special calibration?
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-RF0_RF0-155.pdf - LEGEND has a BSM physics program including DM, backgrounds from Ar39, Ar42, cosmogenic 3H and 68Ge, 
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-IF8_IF0_Guillaume_Giroux-085.pdf - NEWS-G search for 0.1-10 GeV WIMPs with low-A gasses in low-radioactivity Cu in low-210Pb archaeological lead shield. Main background from Pb210 in Cu (Brem photons from Bi210 beta). Future will use 6N electroformed Cu for better purity
%	Yes: https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF3_RF0-CF2_CF0-IF1_IF0_Andrew_Geraci-076.pdf - Optically levitated sensors
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF9_IF8-NF3_NF10-CF1_CF0-145.pdf - direction sensitive DD with noble gas TPCs, NR calibration
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF0-CF0_CF1_JUIJEN_WANG-132.pdf - acrylic scintillators for neutrinos and DM, radiopure acrylic is important. Presumably need to calibrate scintillation efficiency with different dopants (e.g. napthalene). Rn daughter plateout is a major concern
%	Yes: https://www.snowmass21.org/docs/files/summaries/UF/SNOWMASS21-UF4_UF3-NF5_NF6-CF1_CF0-IF3_IF0-CompF2_CompF3-CommF5_CommF0-006.pdf - Very low threshold Ge detectors for LDM and neutrinos, target threshold 0.7 eV to 100 eV, bg rate < 1e-5 cts/keV/kg/yr, need to calibrate charge and phonons, underground crystal growth, leakage current and electrical breakdown issues, backgrounds from electronics, sub keV NR calibration, UMN is using (n,g) for calibration
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-079.pdf - PICO, tonne scale, background from metastable particle-born water droplets eliminated, need <5 nBq/m2 of surface alpha activity due to pileup, low-background active fluid containers other than fused silica, efficient vetoing of muon-induced backgrounds 
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Claudio_Savarese-125.pdf - Low-background SiPMs as low-mass DM detectors with 150 eV threshold in a LNe veto, backgrounds from DCR, DiCT, main R&D challenge to minimize cross talk, 32Si, need low noise, low background electronics, partially-contained gammas and alphas (most will be vetoed)
% 	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF8-CF1_CF0_Hertel-158.pdf - SHe, needs NR calibration to the meV scale, ER down to 19.8 eV 
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF2-CF1_CF0-182.pdf - Phonon sensors for light DM, NR and ER calibration down to O(100 meV), bkgds from dark counts, leakage current, environmental vibrations
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Giovanetti-172.pdf - GADMC, Ar39/UAr, Urania and Aria, neutron backgrounds, veto, low-background SiPM, Kr85 removal, Ar39 < 50 uBq/kg, neutrino floor
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0_Shawn_Westerdale_and_Michael_Clark-133.pdf - Low-threshold noble liquid detectors, sub-keV ER and NR calibration, understand and reduce spurious electron backgrounds, radiopurity to minimize ER backgrounds, Kr85, Ar39, tritium, Rn220, Rn222, radiopure SiPMs and other materials, chemical purity, cosmic ray activation (significant uncertainties), low-energy beta spectrum uncertainties
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0_Eric_Dahl-135.pdf - SBC, vessel materials that won't induce nucleation, NR threshold calibration vs. ER nucleation rate as a function of superheat, scintillation response calibration ~10 keV.
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF0-CF1_CF0_Marshall-110.pdf - Large bandgap directional DM detectors like diamond and silicon carbide, ER/NR calibration down to 1-3 keV, need U/G facilities to avoid cosmic ray exposure of crystals during creation or post-run track/damage anaylsis
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-IF1_IF2_Rouven_Essig-075.pdf - Superconducting Nanostrip Single-Photon Detectors, will require calibration for ERs and NRs below 100 meV
%	Yes: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF0-CF3_CF4_Drlica-Wagner-021.pdf - DD with skipper CCDs, requires low-background and low-noise readout electronics
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-IF2_IF0_Juan_Estrada-080.pdf - OSCURA
%	Yes: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-NF5_NF4-IF8_IF0-CompF0_CompF0-UF2_UF3_Matthew_Szydagis-236.pdf - The Exploitation of Xe Large Scale Detector Technology for a Range of Future Rare Event Physics Searches
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF2_CF7_Andrea_Albert-186.pdf - neV ALPs detected as galactic gammas
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF4-TF1_TF9-032.pdf - Not relevant for DM
%	No: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF2-CF2_CF0_Ankur_Agrawal-149.pdf - wave-like DM
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF2_CF0-IF1_IF0_Aaron_Chou-175.pdf - wave-like DM
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-CompF6_CompF0_A.B._Balantekin-107.pdf - this is about using quantum computation to help with analysis
%	No: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF2_Andrzej_Szelc-145.pdf - all about neutrinos
%	No: https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF0_BDX-076.pdf - beam-dump experiment, doesn't really discuss backgrounds and calibration
% 	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1-TF9_TF0_Katelin_Schutz-127.pdf - theory LOI about cosmological probes benchingmarking and DD
%	No: https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF10_NF0-CF1_CF0-IF1_IF0_Marco_Vignati-061.pdf - more focused on sensor instrumentation 
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0_Yoshiki_Tsunesada-265.pdf - UHECRs, not focused on DM experiment needs
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0_Kristi_L_Engel-227.pdf - Focused on indirect/cosmic probes
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF6_Kristi_L_Engel-231.pdf - Focused on indirect/cosmic probes
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF1_EDV-022.pdf - Focused on theory/cosmic probes
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-IF0_IF7_Aritoki_Suzuki-145.pdf - more instrumentation focused
%	No: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF1-CF4_CF6_Golwala-185.pdf - more cosmology instrumentation
%	No: https://www.snowmass21.org/docs/files/summaries/TF/SNOWMASS21-TF9_TF8-029.pdf - DM pheno
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF2_CF0-IF7_IF0-134.pdf - wave-like DM
%	No: https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF6_RF0_Nhan_Tran-025.pdf - accelerator produced DM
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF7-TF9_TF0_Julian_B._Munoz-209.pdf - theory
%	No: https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF3-NF2_NF3-TF8_TF9_Bibhushan_Shakya-267.pdf - indirect detection
%	No: https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF0-RF6_RF0_Doojin_Kim-056.pdf - axion search, wavelike
%	No: https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF2-177.pdf - focused on instrumentation
%	Yes: https://www.snowmass21.org/docs/files/summaries/RF/SNOWMASS21-RF0_RF0-EF0-CF1-IF0_Jiansong_Gao-086.pdf - Million-pixel Kinetic Inductance Detector Arrays for sub-GeV Light Dark Matter Search

% Ray Bunker
%   https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0-IF1_IF0_Rouven_Essig-089.pdf
%	https://www.snowmass21.org/docs/files/summaries/EF/SNOWMASS21-EF-TOPIC0-004.pdf
%	https://www.snowmass21.org/docs/files/summaries/AF/SNOWMASS21-AF5_AF0-NF2_NF0-RF6_RF0_Vandewater-215.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF7-NF5_NF3_PandaX-073.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Eric_Dahl-099.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Jay_Hyun_Jo-263.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF7_Nilanjan_Banik-207.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF6_CF3_Dickinson-257.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF0-CF1_CF2-TF10_TF0-013.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-NF3_NF10-IF1_IF0-UF3_UF2_SuperCDMS-077.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF0-RF6_RF0-TF8_TF9_Doojin_Kim-070.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF9-111.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF0-CF1_CF0-TF8_TF9_Doojin_Kim-032.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1-TF9_TF8_Vera_Gluscevic,_Kimberly_Boddy-110.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-IF2_IF1_Ben_Mazin-004.pdf
%	https://www.snowmass21.org/docs/files/summaries/TF/SNOWMASS21-TF9_TF0-052.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1_Regina_Caputo-121.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1-TF9_TF8_Vera_Gluscevic,_Kimberly_Boddy-110.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF0_Matthew_Szydagis-174.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF3_Georgia_Karagiorgi-170.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF2-IF1_IF2-102.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1_Stefano_Profumo-007.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF1_CF3_Perez-137.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF0-CF1_CF0-TF8_TF9_Doojin_Kim-049.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF1_IF0-NF10_NF0-CF1_CF2_Golwala-080.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF9_IF8-NF3_NF10-CF1_CF0-145.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF2_Andrzej_Szelc-145.pdf
%	https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-EF6_EF7-NF5_NF6-AF4_AF0_LAA-074.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF1_NF4_Pedro_Ochoa-034.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF2_NF3-RF6_RF0_Athanasios_Hatzikoutelis-160.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF9_NF5-CF1_CF0-IF8_IF0_JNewby-108.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF5_NF4-084.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF4_NF3_Matthew_Strait-090.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF2_IF8-NF10_NF0_Gramellini-137.pdf
%	https://www.snowmass21.org/docs/files/summaries/IF/SNOWMASS21-IF8_IF0-NF10_NF6_Jacob_Zettlemoyer-150.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF-TOPIC0-001.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF10_NF4-CF1_CF0-IF8_IF0-UF1_UF3-137.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF4_Russell_Neilson-017.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF3_NF2-CF7_CF1-TF9_TF8_Katori-073.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF8_NF4-CF1_CF7_Evan_Grohs-174.pdf
%	https://www.snowmass21.org/docs/files/summaries/NF/SNOWMASS21-NF4_NF3-CF1_CF7-TF9_TF11-039.pdf


\end{enumerate}

==> Notes/outline-211210.tex <==


\textbf{Paper Outline}

\begin{enumerate}
    \item Introduction \\\emph{Coordinators}
    \begin{enumerate}
        \item Introduction/motivation/goals
        \item Executive summary
    \end{enumerate}
    \item Calibration \\\emph{Potential Contributors: Eric Dahl, Daniel Egana-Ugrinovic, Rouven Essig, Tali Figueroa, Richard Gaitskell, Scott Hertel, Lauren Hsu, Yoni Kahn, Alexander Kish, Noah Kurinksy, Rafael Lang, Karthik Ramanathan, Alan Robinson, Tarek Saab, Claudio Savarese, Matthew Szydagis, Anthony Villano}
    \begin{enumerate}
        \item Nuclear recoil calibration \\\emph{Lead: Tarek Saab}
        \begin{enumerate}
            \item Internal in situ (e.g. nuclear recoils induced by captures)
            \item External in situ (e.g. photoneutron)
            \item Model calibration far above threshold (e.g. detector linearity, resolution modeling)
            \item Model calibration near threshold (e.g. effects related to quanta production threshold)
            \item Model calibration of low-energy phenomena (e.g. Migdal)
        \end{enumerate}
        \item Electronic recoil calibration at low energies \\\emph{Lead: Karthik Ramanathan?}
        \begin{enumerate}
            \item Internal in situ (e.g. sub-keV calibration sources) 
            \item External in situ - No work needed
            \item Model calibration far above threshold 
            \item Model calibration near threshold 
            \item Model calibration of low-energy phenomena (e.g. plasmon response)
        \end{enumerate}
        \item Coherent excitation calibration at low energies \\\emph{Lead: Scott Hertel}
        \item Material property measurements \\\emph{Lead: Yoni Kahn}
    \end{enumerate}
    \item Backgrounds \\\emph{Potential Contributors: Isaac Arnquist, Susana Cebrian, Laura di Vacri, Rouvin Essig, Cristiano Galbiati, Scott Haselschwardt, Chris Jackson, Noah Kurinsky, Rafael Lang, Ben Loer, Alissa Monte, John Orrell, Jacques Pienaar, Sagar Poudel, Matt Pyle (via IF1 WP), Alan Robinson, Richard Saldanha, Claudio Savarese, Richard Schnee, Dylan Temples}
    \begin{enumerate}
        \item Astrophysical neutrinos (event generation, rates and spectra) \\\emph{Lead: Scott Haselschwardt?}
        \item Cosmogenic neutrons \\\emph{Lead: Sagar Poudel}
        \item Radiogenic neutrons (rate calculations, transport, fast and thermal neutron physics) \\\emph{Lead: Anthony Villano}
        \item Inactive detector material betas/gammas (e.g. U, Th, Pb210, K40) \\\emph{Coordinators}
        \item Surface contaminants (e.g. dust, Pb210, Po210) \\\emph{Lead: Richard Schnee}
        \item Active bulk contaminants, including, e.g., cosmogenically activated isotopes, intrinsic isotopes, contaminants \\\emph{Lead: Susana Cebrian, Eric Miller}
        \item Near-threshold phenomena (these subsections should all be very short)
        \begin{enumerate}
            \item Spurious electrons in noble liquid TPCs \\\emph{Lead: Jingke Xu}
            \item Photo-ionization \\\emph{Lead: Rouven Essig?}
            \item Leakage currents \\\emph{Lead: No lead currently; expect IF1 contribution}
            \item Microfractures \\\emph{Lead: No lead; expect IF1 contribution}
            \item Vibrations \\\emph{Lead: No lead; expect IF1 contribution}
            \item RF-induced pulses \\\emph{Lead: No lead; expect IF1 contribution}
            \item Secondary emission processes \\\emph{Lead: Daniel Egana-Ugrinovic}
            \item Thermal processes \\\emph{Lead: Claudio Savarese}
        \end{enumerate}
    \end{enumerate}
    \item Detector response models/simulations (GEANT4, MCNP, Comsol, NEST, phonon transport) - overlap with WP4. \\\emph{Lead: Matt Szydagis?}
    \begin{enumerate}
        \item Particle transport (e.g. Geant4, MCNP, SRIM, FLUKA) \\\emph{Lead: Alan Robinson? Peter Sorensen? Suerfu?}
        \item Detector response (e.g. NEST, G4CMP) \\\emph{Lead: Mike Kelsey? Noah Kurinsky? Matt Szydagis?}
    \end{enumerate}
    \item Facilities \\\emph{Potential Contributors: Isaac Arnquist, Robert Calkins, Laura di Vacri, Cristiano Galbiati, Jeter Hall, Eric Hoppe, Chris Jackson, Ian Lawson, Ben Loer, Richard Saldanha, Richard Schnee, David Woodward} 
    \begin{enumerate}
        \item Radioassays (how can we address secular disequilibrium?)\\\emph{Lead: Maria Laura di Vacri}
        \item Material needs\\\emph{Lead: Isaac Arnquist}
        \begin{enumerate}
            \item Radiopure material production, understanding and making use of secular disequilibrium
            \item Designing materials that have other favorable properties 
        \end{enumerate}
        \item Material purity infrastructure\\\emph{Lead: Jeter Hall}
        \begin{enumerate}
            \item Underground material production plants (Cu, Ar, etc.) 
            \item Cleaning techniques and facilities, with quantitative verification 
            \item Tools for quantifying material activation in transit
        \end{enumerate}
        \item Underground lab backgrounds, including, e.g., radon \& dust mitigation, gammas and neutrons from cavern walls\\\emph{Lead: David Woodward?}
        \item Software Infrastructure (Radiopurity database, Background Explorer, Assay Request Tool, etc.)\\\emph{Lead: Chris Jackson}
    \end{enumerate}
\end{enumerate}


==> Notes/outline-v0.tex <==
\section{Outline}

\begin{enumerate}
    \item Introduction
    \begin{enumerate}
        \item Introduction/motivation/goals
        \item Executive summary
    \end{enumerate}
    % \item Requirements for different detector types
    % \begin{enumerate}
    %     \item liquid nobles
    %     \item bubble chambers
    %     \item solid state
    % \end{enumerate}
    \item Calibration 
    \begin{enumerate}
        \item Nuclear recoil calibration 
        \begin{enumerate}
            \item In situ
            \item Ex situ, including detection of, e.g., Migdal effect, Bremsstrahlung, etc.
        \end{enumerate}
        \item Electronic recoil calibration at low energies
        \begin{enumerate}
            \item In situ
            \item Ex situ, including detection of, e.g., plasmon resonance
        \end{enumerate}
        \item Coherent excitation calibration at low energies
        \begin{enumerate}
            \item In situ
            \item Ex situ
        \end{enumerate}
        % \item Calibration for indirect detection?
        % \item Detecting low-energy phenomena like Migdal effect, Bremsstrahlung, plasmon resonance, coherent photonuclear scattering
        \item Detector response models/simulations (GEANT4, MCNP, Comsol, NEST, phonon transport)
        \item Anything else for specific detection techniques (e.g. directional detectors, indirect detection)?
    \end{enumerate}
    \item Backgrounds 
    \begin{enumerate}
        \item Astrophysical neutrinos (event generation, rates and spectra)
        \item Cosmogenic neutrons 
        \item Radiogenic neutrons (rate calculations, transport, fast and thermal neutron physics)
        % \item Underground environmental backgrounds (gammas, neutron, Rn and dust in air)
        \item Inactive detector material betas/gammas (e.g. U, Th, Pb210, K40)
        \item Surface contaminants (e.g. dust, Pb210, Po210)
        \item Active bulk contaminants, including, e.g., cosmogenically activated isotopes, intrinsic isotopes, contaminants
        \item Near-threshold phenomena 
        \begin{enumerate}
            \item Spurious electrons in noble liquid TPCs 
            \item Photo-ionization 
            \item Leakage currents 
            \item Microfractures 
            \item Vibrations 
            \item RF-induced pulses
            \item Secondary emission processes
            \item Thermal processes
        \end{enumerate}
        % \item Spurious electron backgrounds (e.g. dark rates, leakage currents, photo-ionization)
        % \item Secondary emission processes
        % \item Instrumental noise (microfractures, vibrations, RF induced pulses)
        \item Anything for indirect detection?
    \end{enumerate}
    \item Facilities
    \begin{enumerate}
        \item Radioassays
        \item Underground material production plants (generalize to include low-activity argon production, e.g.?)
        \item Underground lab backgrounds, including, e.g., radon \& dust mitigation, gammas and neutrons from cavern walls
        \item Software Infrastructure (Radiopurity database, Background Explorer, Assay Request Tool, etc.)
    \end{enumerate}
\end{enumerate}
